Learning Dependencies in Distributed Cloud Applications to Identify and Localize Anomalies

Operation and maintenance of large distributed cloud applications can quickly become unmanageably complex, putting human operators under immense stress when problems occur. Utilizing machine learning for identification and localization of anomalies in such systems supports human experts and enables fast mitigation. However, due to the various inter-dependencies of system components, anomalies do not only affect their origin but propagate through the distributed system. Taking this into account, we present Arvalus and its variant D-Arvalus, a neural graph transformation method that models system components as nodes and their dependencies and placement as edges to improve the identification and localization of anomalies. Given a series of metric KPIs, our method predicts the most likely system state - either normal or an anomaly class - and performs localization when an anomaly is detected. During our experiments, we simulate a distributed cloud application deployment and synthetically inject anomalies. The evaluation shows the generally good prediction performance of Arvalus and reveals the advantage of D-Arvalus which incorporates information about system component dependencies.

==> sections/background.tex <==
% \section{Background}
% \label{sec:background}

% \subsection{Microservices}
% \label{sec:background_microservices}
% The term "Microservices" describes a design paradigm for software applications based on specific characteristics.
% It is widely applied in different domains where it complements or replaces monolithic applications~\cite{dragoni2017microservices}.
% Thereby, the application is split into independent and self-contained services with defined communication APIs.
% Each Microservice is deployed individually, which enables horizontal scalability each service.
% Such collections of microservices are referred to as microservice architectures (MSAs).
% The often positively discussed characteristics of mircroservices~\cite{dragoni2017microservices} are introducing additional problems~\cite{Wu2020microRCA}.
% The distribution of services entails increased network communication.
% Thus, network problems have a high impact on the service quality.
% The monitoring of MSAs is complex.
% KPIs from hundreds to thousands of services, each consisting of one or more running processes, has to be collected.
% Furthermore, the heterogeneity of services (e.g. written in different programming languages) requires flexible monitoring solutions.
% Another key challenge is the detection and localization of anomalies and failures, since they propagate and affect several services at once.
% Therefore, the operation and maintenance of MSAs is an active field of research.




==> sections/evaluation_dataset.tex <==
\subsection{Dataset Construction}
\label{sec:evaluation_dataset}

% From an external perspective, we can view the state of all systems at any point in time.
% For the dataset construction, ...
%We extract subseries of the raw multivariate time series in order to create data samples.
% As implied in \autoref{sec:approach_prel}, 
% we can extract subseries of the multivariate time series by moving along the temporal dimension with a window width $w$ and a stride $s$.
We utilize the previously described KPI simulation to create a multivariate time series for each system component.
Further, we employ a sliding window of $20$ samples with a stride of $20$ to extract subseries that are used to construct the node feature vectors.
% The latter effectively controls the amount of information incorporated into each sample.
Each subseries of a system component is labeled with two labels.
Firts by a 

Each sample is further enriched by several properties, i.e. 1) the extracted \emph{subseries} of all systems at the respective point in time, 2) the \emph{dependencies} between all systems, 3) the information about the state of each system encoded in so-called \emph{node labels}, 4) the randomly chosen \emph{target metric} of the respective target node subject to an anomaly injection, and 5) a randomly chosen subset of $3\leq k \leq 7$ neighbors plus target metrics from all neighbors of the respective target node.
% \begin{itemize}
%     \item \verb|Subseries|: The extracted subseries of all systems at the respective point in time.
%     \item \verb|Dependencies|: The possibly unidirectional dependencies between all systems.
%     \item \verb|Node labels|: The information about the state of each system, encoded in so-called labels.
%     \item \verb|Target metric|: For each sample, we randomly choose the metric subject to an anomaly injection. 
%     \item \verb|Neighbors|: For each sample, we randomly choose a subset of $3\leq k \leq 7$ neighbors plus target metrics from all neighbors of the respective target node. 
% \end{itemize}
% We enrich each sample with the following information:
% \begin{itemize}
%     \item \verb|Subseries|: The extracted subseries of all systems at the respective point in time.
%     \item \verb|Dependencies|: The possibly unidirectional dependencies between all systems.
%     \item \verb|Node labels|: The information about the state of each system, encoded in so-called labels.
%     \item \verb|Target metric|: For each sample, we randomly choose the metric subject to an anomaly injection. 
%     \item \verb|Neighbors|: For each sample, we randomly choose a subset of $3\leq k \leq 7$ neighbors plus target metrics from all neighbors of the respective target node. 
% \end{itemize}
Moreover, we alter the captured data in each sample to account for the unsteady nature of dynamic and real systems. We randomly choose from three scenarios with probabilities 70\%, 20\% and 10\%:
\begin{itemize}
    \item \verb|Local|: While system node $i$ experiences an anomalous behavior, all other nodes are normal.
    \item \verb|Neighborhood|: While system node $i$ reveals a miscellaneous state, its respective $k$ neighbors are subject to an injection of the actual anomaly.
    \item \verb|Adversary|: While system node $i$ experiences an anomalous behavior, its respective $k$ neighbors are subject to an injection of the corresponding adversary anomaly.
\end{itemize}
The original node labels are updated according to these alterations.
During identification and localization, the respective models will be trained to predict the node labels.

% The experiment described in \autoref{sec:evalation_experiment} had a total duration of approximately 2 days. 
% KPIs were monitored for each system, thus from an external perspective, we can view the state of all systems at any point in time.
% For the dataset construction, we extract subseries of the raw multivariate time series in order to create data samples. 
% As visualized in \autoref{fig:ts_slicing}, we can extract slices of the multivariate time series by moving along the temporal dimension with a window width $w$ and a stride $s$. 
% For our experiments, we choose a stride $s=10s$ and three different window widths $w\in \{10s,25s,50s\}$, which effectively leads to three datasets, each with a different amount of context available per sample. 
% Moreover, each created data sample contains the extracted subseries of all systems at the respective point in time, while also keeping track of the corresponding labeling, as depicted in \autoref{sec:background_ts}. 
% Whenever a subseries contains less observations than expected, e.g. due to a drop in the envisioned monitoring frequency, we use upsampling to account for that. 
% The system dependencies are preserved in each sample as well. 
% We enrich each sample with the following information:
% \begin{itemize}
%     \item node labels: Information about the state of each system, encoded in so-called labels.
%     \item graph label: Due to the nature of our experiment conducted in \autoref{sec:evalation_experiment}, anomalies were injected in a sequential manner, which is why for any sample, all systems are labeled normal, with at most one being labeled anomalous. This label is assigned to the sample.
% \end{itemize}
% For our evaluation, we are only interested in anomaly samples. Thus, we exclude all samples with graph labels indicating a normal state across all systems.
% During classification, the respective models will be trained to predict the node labels.

% \begin{figure}
%     \centering
%     \includegraphics[trim=0 80 40 190, clip,keepaspectratio,width=\columnwidth]{graphics/evaluation/ts_slicing.pdf}
%     \caption{A window is moved along the temporal dimension of a multivariate time series with a configurable stride while subseries are extracted.}
%     \label{fig:ts_slicing}
% \end{figure}

% \begin{table}[ht]
% \centering
% \caption{Datasets}
% \small
%     \begin{tabular}[t]{l||c|c|c}
%         \toprule
%         & \textbf{Dataset 1} & \textbf{Dataset 2} & \textbf{Dataset 3}\\
%         \midrule
%         Stride & 10s & 10s & 10s\\
%         Window Width & 10s & 25s & 50s\\
%         \#Data Samples & 9.915 & 9.906 & 9.915 \\
%         \midrule
%         \#Parameters Baseline & 7.719 & 12.519 & 20.519 \\
%         \#Parameters \emph{Arvalus} & 7.703 & 12.503 & 20.503 \\
%         \bottomrule
%     \end{tabular}
% \label{tbl:evaluation_dataset}
% \end{table}

==> sections/introduction_OLD.tex <==
\section{Introduction}
\label{sec:introduction}

The rapid evolution of IT systems enables the development of novel applications and services in a variety of fields like medicine, autonomous transportation or manufacturing.  
Requirements of high availability and minimal latency together with general growth in distribution, size and complexity of these systems aggravate their operation and maintenance. Nowadays, the size of cloud systems is no longer manageable by humans alone. The increase of automation is therefor a logical consequence.

While many existing automated techniques can successfully increase the availability of distributed systems due to prevention of component outages, a hardware or software component is potentially also able to exhibit an undesired behavior without leading to a total outage. Such anomalies and methods for dealing with them are subject of current research. One specific research direction in that area utilizes methods from machine learning for operation and maintenance of IT systems~\cite{dang2019aiops,gulenkoa2016system}.
It includes methods for anomaly detection, anomaly localization as well as recommendation and auto-remediation methods to execute actions and transfer anomalous system components back to a normal operation state. Therefore, monitoring systems are employed to collect key performance indicators (KPIs) like network latency and throughput or system resource utilization from relevant IT system components.
Significant research work is done on methods for anomaly detection~\cite{nedelkoski2019anomaly,wetzig2019unsupervised} and root cause analysis~\cite{wu2020microrca}.

However, existing solutions mostly fail to propose a holistic approach for an automated remediation execution, mainly due to two reasons. On the one hand, they often focus on unsupervised methods, and although this is important to enable the detection of previously unseen anomalies, it imposes suboptimal implications. A generic anomaly class that summarizes all types of anomalies either implies actions that are able to remediate all anomaly types or pushes the responsibility for selecting an appropriate remediation to a subsequent instance - usually a human expert. 
Therefore, we propose a method to recognize reoccurring anomalies by training a classification model. On the other hand, methods suited for a certain system likely encounter difficulties when transferred to another system. This is either because a static dimensionality of the input data is assumed or the method is simply not able to generalize. On top of that, the effects of system interactions and their dependencies often remain unconsidered, because the undesired behavior is only locally searched for.

Utilizing system metric data like CPU utilization, allocated memory or disk I/O statistics of various interacting systems, expressing their metrics as multivariate time series, extracting slices of these time series and modeling each observed variable and its extracted features as a node with corresponding node features in a reasonably connected global graph, our model is able to identify anomaly type specific patterns and to assign respective anomaly labels to those. By modeling the diverse KPIs of various source systems as a global graph, our method can exploit inter-system relations and dependencies, thus incorporating more knowledge into the process of decision making. Moreover, it has the advantage of being invariant to changing dimensionalities of input data as well as the total number of modeled systems. Currently proposed anomaly classification methods assume a static dimensionality of input data, which is usually not the case for IT systems, which undergo frequent changes due to software updates, hardware modernization, etc.
To enable the automation of anomaly remediation, we propose a novel anomaly type classification solution, which is utilized to detect reoccurring anomaly types while retaining information about the localization of specific anomalies. 
To this end, our proposed model architecture ARVALUS utilizes a novel graph neural network architecture to exploit several systems and their KPIs modeled as a single graph both in the spatial and temporal dimension.

The rest of the paper is structured as followed. 
In \autoref{sec:approach}, we describe the preliminaries for our approach and present ARVALUS in detail. 
A consolidation of the conducted evaluation is given in \autoref{sec:evaluation}, encompassing the hyper-parametrization and training setup, the testbed and experiment design as well as the results of classification and localization of anomalies and their discussion. 
An excerpt of related approaches is presented in \autoref{sec:relatedWork} capturing the state of the art. 
Lastly, \autoref{sec:conclusion} concludes this paper and gives an outlook for future work.  








